No Reason for No Supervision: Improved Generalization in Supervised Models

We consider the problem of training a deep neural network on a given classification task, e.g., ImageNet-1K (IN1K), so that it excels at both the training task as well as at other (future) transfer tasks. These two seemingly contradictory properties impose a trade-off between improving the model's generalization and maintaining its performance on the original task. Models trained with self-supervised learning tend to generalize better than their supervised counterparts for transfer learning; yet, they still lag behind supervised models on IN1K. In this paper, we propose a supervised learning setup that leverages the best of both worlds. We extensively analyze supervised training using multi-scale crops for data augmentation and an expendable projector head, and reveal that the design of the projector allows us to control the trade-off between performance on the training task and transferability. We further replace the last layer of class weights with class prototypes computed on the fly using a memory bank and derive two models: t-ReX that achieves a new state of the art for transfer learning and outperforms top methods such as DINO and PAWS on IN1K, and t-ReX* that matches the highly optimized RSB-A1 model on IN1K while performing better on transfer tasks. Code and pretrained models: https://europe.naverlabs.com/t-rex

==> float/fig_grad_similarity.tex <==
\begin{wrapfigure}[10]{R}{0.30\linewidth}
    \begin{center}
    \input{float/tikz_gradient_stat.tex}
    \caption{
        Average cosine similarity between gradient vectors of class weights $\nabla_{\netw_c}\lossce$.
    }
    \label{fig:grad_similarity}
    \end{center}
\end{wrapfigure}

==> float/fig_multicrop_localnumber.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{res/multicrop_localnumber_a.pdf}
        \caption{multi-crop without using a projector}
        \label{fig:multicrop_noproj}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{res/multicrop_localnumber_b.pdf}
        \caption{multi-crop using a projector}
        \label{fig:multicrop_proj}
    \end{subfigure}
    \caption{
        {\bf Impact of the number of local crops} on \imnet performance (Top-1 Accuracy) and mean transfer Accuracy (log odds) over the 13 transfer datasets.
        \textit{Left:} Varying the number of global crops without using a projector head.
        \textit{Right:} Varying the number of hidden layers in the projector head.
    }
    \label{fig:multicrop_localnumber}
\end{figure}
